A Comparative Study of Machine Learning Algorithms for Anomaly Detection in Industrial Environments: Performance and Environmental Impact

In the context of Industry 4.0, the use of artificial intelligence (AI) and machine learning for anomaly detection is being hampered by high computational requirements and associated environmental effects. This study seeks to address the demands of high-performance machine learning models with environmental sustainability, contributing to the emerging discourse on 'Green AI.' An extensive variety of machine learning algorithms, coupled with various Multilayer Perceptron (MLP) configurations, were meticulously evaluated. Our investigation encapsulated a comprehensive suite of evaluation metrics, comprising Accuracy, Area Under the Curve (AUC), Recall, Precision, F1 Score, Kappa Statistic, Matthews Correlation Coefficient (MCC), and F1 Macro. Simultaneously, the environmental footprint of these models was gauged through considerations of time duration, CO2 equivalent, and energy consumption during the training, cross-validation, and inference phases. Traditional machine learning algorithms, such as Decision Trees and Random Forests, demonstrate robust efficiency and performance. However, superior outcomes were obtained with optimised MLP configurations, albeit with a commensurate increase in resource consumption. The study incorporated a multi-objective optimisation approach, invoking Pareto optimality principles, to highlight the trade-offs between a model's performance and its environmental impact. The insights derived underscore the imperative of striking a balance between model performance, complexity, and environmental implications, thus offering valuable directions for future work in the development of environmentally conscious machine learning models for industrial applications.

==> tables/table_performance_cross_validation.tex <==
% \usepackage{caption}
\begin{table}[htbp]
\centering
\captionsetup{labelformat=empty}
\caption{Machine Learning Algorithms Performance Comparison }
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l}
~        & Model                           & Accuracy & AUC    & Recall & Prec.  & F1     & Kappa  & MCC    & F1 Macro & TT (Sec)  \\ 
\hline
rf       & Random Forest Classifier        & 0.9997   & 0.9687 & 0.9997 & 0.9997 & 0.9997 & 0.8916 & 0.8961 & 0.9335   & 9.579     \\
dt       & Decision Tree Classifier        & 0.9995   & 0.9084 & 0.9995 & 0.9995 & 0.9995 & 0.8148 & 0.8165 & 0.9101   & 2.269     \\
et       & Extra Trees Classifier          & 0.9997   & 0.9737 & 0.9997 & 0.9996 & 0.9996 & 0.8618 & 0.8707 & 0.7686   & 5.809     \\
lda      & Linear Discriminant Analysis    & 0.9993   & 0.9051 & 0.9993 & 0.9996 & 0.9994 & 0.7558 & 0.7577 & 0.7303   & 1.507     \\
ada      & Ada Boost Classifier            & 0.9996   & 0.9796 & 0.9996 & 0.9995 & 0.9995 & 0.8318 & 0.8405 & 0.6827   & 5.147     \\
lr       & Logistic Regression             & 0.9996   & 0.997  & 0.9996 & 0.9996 & 0.9996 & 0.8452 & 0.855  & 0.6679   & 14.001    \\
svm      & SVM - Linear Kernel             & 0.9995   & 0      & 0.9995 & 0.9994 & 0.9994 & 0.8034 & 0.8117 & 0.6313   & 1.662     \\
ridge    & Ridge Classifier                & 0.9996   & 0      & 0.9996 & 0.9995 & 0.9995 & 0.8362 & 0.8484 & 0.6265   & 0.945     \\
lightgbm & Light Gradient Boosting Machine & 0.9977   & 0.8347 & 0.9977 & 0.9988 & 0.9982 & 0.4643 & 0.4916 & 0.5517   & 5.172     \\
nb       & Naive Bayes                     & 0.9685   & 0.9961 & 0.9685 & 0.9987 & 0.9829 & 0.0734 & 0.1886 & 0.3953   & 0.732     \\
qda      & Quadratic Discriminant Analysis & 0.9797   & 0.9753 & 0.9797 & 0.9986 & 0.9886 & 0.1047 & 0.2223 & 0.364    & 0.875     \\
dummy    & Dummy Classifier                & 0.9986   & 0.5    & 0.9986 & 0.9973 & 0.998  & 0      & 0      & 0.3331   & 0.901    
\end{tabular}
\end{table}
